Storywrangler: A massive exploratorium for sociolinguistic, cultural, socioeconomic, and political timelines using Twitter

In real-time, social media data strongly imprints world events, popular culture, and day-to-day conversations by millions of ordinary people at a scale that is scarcely conventionalized and recorded. Vitally, and absent from many standard corpora such as books and news archives, sharing and commenting mechanisms are native to social media platforms, enabling us to quantify social amplification (i.e., popularity) of trending storylines and contemporary cultural phenomena. Here, we describe Storywrangler, a natural language processing instrument designed to carry out an ongoing, day-scale curation of over 100 billion tweets containing roughly 1 trillion 1-grams from 2008 to 2021. For each day, we break tweets into unigrams, bigrams, and trigrams spanning over 100 languages. We track n-gram usage frequencies, and generate Zipf distributions, for words, hashtags, handles, numerals, symbols, and emojis. We make the data set available through an interactive time series viewer, and as downloadable time series and daily distributions. Although Storywrangler leverages Twitter data, our method of extracting and tracking dynamic changes of n-grams can be extended to any similar social media platform. We showcase a few examples of the many possible avenues of study we aim to enable including how social amplification can be visualized through 'contagiograms'. We also present some example case studies that bridge n-gram time series with disparate data sources to explore sociotechnical dynamics of famous individuals, box office success, and social unrest.

==> bin/rename <==
#!/usr/bin/perl

$usage = "rename text1 text2 file [files...]

swap text1 for text2 in file names
whenever text1 is found.

swaps only the first instance.

rudimentary first version: use only for static text.
";

$pattern1 = $ARGV[0];
$pattern2 = $ARGV[1];

foreach $filename (@ARGV[2..$#ARGV]) {
    if ($filename =~ m/$pattern1/) {
	($newfilename = $filename) =~ s/$pattern1/$pattern2/g;
	print "renaming $filename as $newfilename...\n";
	`mv "$filename" "$newfilename"`;
    }
}


==> story-wrangler-revtex4.settings.tex <==
\newcommand{\filenamebase}{story-wrangler}


==> story-wrangler.biblio.tex <==
\bibliography{\filenamebase}


==> story-wrangler.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}



==> story-wrangler.outtakes.tex <==
people can be present or remote

potentially greatly increases the observer base.


Although Twitter as a single social media outlet is a
non-representative sub-sample of the whole human population for many
reasons~\cite{mellon2017twitter,perrin2019share},

The StoryWrangler instrument reveals one of our various attempts to
capture these modern sociolinguistic phenomena.


from diverse sources,

We can , our data set allows researchers to explore transitions in social amplification
by reconstructing $n$-gram Zipf distributions with a tunable fraction of retweets.


Twitter also  ones engaged in deliberate misinformation.


for political figures and celebrities.  major events are represented
Twitter does track major news events 
the general trend of popular culture,
political events~\cite{steinert2015online},
and natural disasters~\cite{pickard2011time,gao2011harnessing,lampos2010tracking,Culotta2010towards}.

Twitter is a real-time source of information annotating the global
collective attention broadcast on the platform.

The immediacy of Twitter means that we can track storylines in real time.


When is the $n$-gram
Which species are present in an ecological system,
which kinds of jobs does a city

When does a species become part of an ecology,
a type of employment exist in a city
Lexicographers' pursuit of the first use of words and phrases~\cite{OED}.

And 
Which kinds of atoms are present in higher-order life forms,
which 


\paragraphnutshell{Intro on corpora, history}


Shorn of popularity


an $n$-gram appears in a text.

We determine how frequently


And then we reach the highest level of popularity,
as measured by how often an $n$-gram is read.


\begin{figure*}[tp!]
  \centering	
    \includegraphics[width=0.67\textwidth]{figures/local/2020-05-21chart.pdf}
  \caption{
    \todo{Add caption}
  }
  \label{fig:}
\end{figure*}



Retrieving None: 1gram -- '2012'
Top rank: 26.0 -- 2011-12-31
Retrieving None: 1gram -- '2014'
Top rank: 22.0 -- 2013-12-31
Retrieving None: 1gram -- '2016'
Top rank: 24.0 -- 2016-01-01
Retrieving None: 1gram -- '2018'
Top rank: 13.0 -- 2018-01-01
Retrieving English: 1gram -- 'Christmas'
Top rank: 11.0 -- 2012-12-25
Retrieving Italian: 1gram -- 'Pasqua'
Top rank: 21.0 -- 2017-04-16
Retrieving Portuguese: 1gram -- 'eleição'
Top rank: 138.0 -- 2018-10-28
Retrieving Swedish: 1gram -- 'sommar'
Top rank: 210.0 -- 2014-06-30
Retrieving English: 1gram -- 'Olympics'
Top rank: 135.0 -- 2012-07-27
Retrieving English: 2gram -- 'World Cup'
Top rank: 5.0 -- 2014-07-13
Retrieving English: 2gram -- 'Super Bowl'
Top rank: 3.0 -- 2014-02-02
Retrieving English: 1gram -- 'Higgs'
Top rank: 889.0 -- 2012-07-04
Retrieving English: 1gram -- '#AlphaGo'
Top rank: 4533.0 -- 2016-03-13
Retrieving English: 2gram -- 'gravitational waves'
Top rank: 487.0 -- 2016-02-11
Retrieving English: 1gram -- 'CRISPR'
Top rank: 13832.5 -- 2018-11-26
Retrieving English: 2gram -- 'black hole'
Top rank: 32.0 -- 2019-04-10
Retrieving Portuguese: 2gram -- 'Cristiano Ronaldo'
Top rank: 21.0 -- 2018-06-15
Retrieving English: 2gram -- 'Donald Trump'
Top rank: 6.0 -- 2016-11-09
Retrieving Italian: 2gram -- 'Papa Francesco'
Top rank: 46.0 -- 2013-03-13
Retrieving English: 1gram -- 'cholera'
Top rank: 3757.0 -- 2010-10-24
Retrieving English: 1gram -- 'Ebola'
Top rank: 131.0 -- 2014-10-02
Retrieving English: 1gram -- 'Zika'
Top rank: 1229.0 -- 2016-02-02
Retrieving English: 1gram -- 'coronavirus'
Top rank: 44.0 -- 2020-03-12
Retrieving Arabic: 1gram -- 'غزة'
Top rank: 38.0 -- 2010-05-31
Retrieving French: 1gram -- 'Libye'
Top rank: 108.0 -- 2011-03-19
Retrieving Turkish: 1gram -- 'Suriye'
Top rank: 59.0 -- 2019-10-13
Retrieving Ukrainian: 1gram -- 'Росія'
Top rank: 32.0 -- 2014-03-03
Retrieving Arabic: 1gram -- 'ثورة'
Top rank: 72.0 -- 2011-02-12
Retrieving English: 1gram -- 'Occupy'
Top rank: 901.0 -- 2011-10-15
Retrieving English: 3gram -- 'Black Lives Matter'
Top rank: 4.0 -- 2020-06-02
Retrieving English: 1gram -- 'Brexit'
Top rank: 137.0 -- 2016-06-24
Retrieving English: 1gram -- '#MeToo'
Top rank: 461.0 -- 2017-10-16

==> story-wrangler.pacs.tex <==
\pacs{89.65.-s,89.75.Da,89.75.Fb,89.75.-k}

%% 89.65.-s	Social and economic systems
%% 89.75.Da	Systems obeying scaling laws
%% 89.75.Fb	Structures and organization in complex systems
%% 89.75.-k	Complex systems (for complex chemical systems, see 82.40.Qt; for biological complexity, see 87.18.-h)


